Infusing Environmental Captions for Long-Form Video Language Grounding

In this work, we tackle the problem of long-form video-language grounding (VLG). Given a long-form video and a natural language query, a model should temporally localize the precise moment that answers the query. Humans can easily solve VLG tasks, even with arbitrarily long videos, by discarding irrelevant moments using extensive and robust knowledge gained from experience. Unlike humans, existing VLG methods are prone to fall into superficial cues learned from small-scale datasets, even when they are within irrelevant frames. To overcome this challenge, we propose EI-VLG, a VLG method that leverages richer textual information provided by a Multi-modal Large Language Model (MLLM) as a proxy for human experiences, helping to effectively exclude irrelevant frames. We validate the effectiveness of the proposed method via extensive experiments on a challenging EgoNLQ benchmark.

==> 2_prior.tex <==
\section{Related Work}
\label{sec:related}
% === Tips === 
% - Use PRESENT tense to describe related work.
% - Avoid a laundry list of paper. A et al. propose X. B et al. propose Y. Instead, tell a story within each topic and cite relevant papers along the way.
% - Citations is NOT nouns. You cannot start a sentence with a citation (e.g. [1] proposes...). Your sentences should still make sense when you remove all the citations.
% - Do not just list related work. "Relate" them with this work. What's similar? What's different?
% - Example of citation: Huang~\etal~\cite{Huang-CVPR-2015}. The symbol "~" avoids breaking the words into different lines.

% === General structure within each topic ===
% (1) Introducing this topic. What's the input/output?

% (2) What other people have done in this topic?
% [Example] (Do not list! Organize!) 
% - Generative Adversarial Networks (GANs) [15, 62] have achieved impressive results in image generation [5, 37], image editing [65], and representation learning [37, 42, 35]. Recent methods adopt the same idea for conditional image generation applications, such as text2image [39], image inpainting [36], and future prediction [34], as well as to other domains like videos [53] and 3D data [56]. 

% (3) How our work RELATES to the papers in this topic? (Focus on "we", "our work", "our main focus")
% [Example] (for similar ideas)
% - Our work builds upon XXX and tackle the problem of XXX.
% - We use  XXX
% - In this work, we introduce a similar loss to XXX
% 
% [Example] (for different ideas)
% - In contrast to existing methods~\cite{XXX} that do XXX, we do XXX. We show that XXX ...
% - Existing approaches did XXX. Our main focus, on the other hand, is XXX
% - Unlike the above approaches, our formulation does not rely on XXX

% Before revision by Jinwoo
% \textbf{Long-Form video-language grounding.} Long-Form video-language grounding (\lfvlg{}) have become a vibrant research area with the advent of long-term video datasets~\cite{Soldan_2022_CVPR, ZhXuCoCVPR18, lei2021detecting, grauman2022ego4d}. Existing approaches include i) Structural approaches~\cite{Cao_2023_CVPR, hou2023cone, hou2023groundnlq, Mun_2020_CVPR} ii) additional information infusion~\cite{ramakrishnan2023naq, Croitoru_2023_ICCV, nagarajan2023egoenv} iii) multi-task learning~\cite{Zheng_2022_CVPR, zhanghelpinghand, di2023groundvqa, jang2023knowing}. EgoEnv\cite{nagarajan2023egoenv} suggested modeling the physical environment, its approach requires simulation construction, making it less accessible. In this work, We provides comprehensive details about the environment and this can help to reduce search space without simulation construction or proposals.

% After revision by Jinwoo
% \paragraph{Long-Form Video-Language Grounding.} 
\paragraph{Long-form video-language grounding (\lfvlg{}).}
Recently, \lfvlg{} has become an active research area with the introduction of long-form video datasets~\cite{Soldan_2022_CVPR, ZhXuCoCVPR18, lei2021detecting, grauman2022ego4d}. 
%
Existing approaches include proposal generation~\cite{Cao_2023_CVPR, hou2023cone, hou2023groundnlq, Mun_2020_CVPR}, multi-task learning~\cite{Zheng_2022_CVPR, zhanghelpinghand, di2023groundvqa, jang2023knowing}, additional information injection with data augmentation~\cite{ramakrishnan2023naq, Croitoru_2023_ICCV} and physical environment modeling~\cite{nagarajan2023egoenv}.
%
We also propose to utilize additional information. 
%
In contrast to prior works, we leverage high-quality knowledge from a multi-modal large language model to provide comprehensive details about the environment, thereby effectively reducing the search space. 
%
The most relevant prior work is EgoEnv~\cite{nagarajan2023egoenv}, which constructs a 3D environment.
%
Compared to EgoEnv, the proposed method is more accessible because \jw{describe why}. \sy{our method doesn't need additional data like simulation data for training.}



% Before revision by Jinwoo
% \textbf{Multi-modal Large Language Models.} Multi-modal Large Language Models(MLLMs)~\cite{li2023llavamed, liu2024llavanext, liu2024visual, liu2023improvedllava,zhang-etal-2023-video, lin2023video,li2022blip, li2023blip2, instructblip, ren2023timechat, maaz2023videochatgpt} built upon open-source LLMs~\cite{radford2018improving, radford2019language, NEURIPS2020_1457c0d6,
% touvron2023llama, touvron2023llama2, jiang2023mistral, jiang2024mixtral, vicuna2023, alpaca} have demonstrated superior zero-shot performance in various video tasks, including needle-in-a-haystack and VideoQA. MLLMs can generate comprehensive explanations encompassing object detection and action recognition, even from short-term videos or single frames. Despite this, it is challenging for MLLMs to perform VLG~\cite{ren2023timechat, feng2023llm4vg, wang2024lifelongmemory, wang2023egocentric}, though tuned with instructions. Rather than applying MLLMs directly to the VLG task, we employ MLLMs to extract detailed environmental information from the video.

% After revision by Jinwoo
\paragraph{Multi-modal large language models (MLLMs).} 
%
MLLMs~\cite{li2023llavamed, liu2024llavanext, liu2024visual, liu2023improvedllava, zhang-etal-2023-video, lin2023video, zhang2023llava, li2022blip, li2023blip2, instructblip, ren2023timechat, maaz2023videochatgpt} built upon open-source LLMs~\cite{radford2018improving, radford2019language, NEURIPS2020_1457c0d6,
touvron2023llama, touvron2023llama2, jiang2023mistral, jiang2024mixtral, vicuna2023, alpaca} have demonstrated remarkable zero-shot performance in various video tasks, such as video question answering, object detection, ~\cite{zhang2023llava} and action recognition~\cite{yan2023videococa}.
%
Despite their great capabilities in many tasks, MLLMs struggles in VLG tasks~\cite{ren2023timechat, feng2023llm4vg, wang2024lifelongmemory, wang2023egocentric} \jw{why?}\hg{Timechat's charades performace}
\sy{Despite their great capabilities in many tasks, MLLMs like TimeChat~\cite{ren2023timechat} exhibit relatively low performance in VLG tasks, achieving only an R1@0.5 performance of 32.2\% on Charades-STA, indicating the difficulty of directly solving VLG with MLLMs.}
%
In this work, we employ an MLLM as an environmental knowledge extractor to effectively reduce the search space, rather than applying MLLMs directly to solve the VLG task.



% Before revision by Jinwoo
% \textbf{Information Retrieval.} Previously, text models have been employed to find specific information within long documents. In particular, Sentence-BERT \cite{reimers-gurevych-2019-sentence, reimers-2020-multilingual-sentence-bert, thakur-2020-AugSBERT} have shown improved performance over cross-encoders \cite{gao2021rethink, he2023debertav3, nogueira2020passage, clark2020electra} because they do not require joint computation between the document and the query, thereby reducing computational complexity. A key difference between VLG and information retrieval is that information retrieval typically does not require distinguishing between different contexts within a single document, whereas the VLG task involves differentiating between various environments within in-video clips, not inter-video clips \cite{linegocentric}. we extend the process of obtaining fragmented information by leveraging environmental text information to differentiate between various in-video clips.

% After revision by Jinwoo
\paragraph{Information retrieval.} 
In information retrieval tasks, Sentence-BERT families \sy{ -> dual-encoders}~\cite{reimers-gurevych-2019-sentence, reimers-2020-multilingual-sentence-bert, thakur-2020-AugSBERT} \mj{better to say `dual-encoders or bi-encoders' than `Sentence-BERT families'} have shown improved performance \sy{ -> efficiency} over cross-encoders~\cite{gao2021rethink, he2023debertav3, nogueira2020passage, clark2020electra} because they do not require joint computation \jw{computation or performance?} between the document and the query, thereby reducing computational complexity. 
\mj{not sure if mentioning the advantage of dual-encoders over cross-encoders is really necessary or relevant to our work.}
%
In a \lfvlg{} task, a model also needs to retrieve a moment most relevant to an input query.
%
A key difference between \lfvlg{} and information retrieval is the need for context discrimination.
%
Information retrieval tasks typically do not require distinguishing between different contexts within an input document.
\mj{not sure if this is true. information retrievers (or dense retrievers) are trained to "distinguish relevant documents from all irrelevant ones in the entire corpus (see the introduction of https://arxiv.org/pdf/2007.00808)".}
%
In contrast, \lfvlg{} involves discriminating various visual contexts, referred to as \emph{environments}, within an input video.
%
We leverage an MLLM to provide environmental information, \ie detailed captions, to discriminate various contexts and thereby reduce the search space.



% \paragraph{Contrastive learning.} 
% self-supervised learning을 위해 contrastive loss를 사용하는 것을 시도한 논문들이 많이 있다.
% 특히 ego4d dataset에서는 EgoNCE loss를 사용한 논문이 많다. (egovlpv1, egovlpv2, 등등등)
% \lfvlg{} involves discriminating various visual contexts, referred to as \emph{environments}, within an input video.
% 하지만, 이 egonce loss는 withan an input video 상이 아닌 서로 다른 비디오를 구분하기 위한 loss에 특화가 되어있다. 또한, 카메라 착용자와 상호작용하는 object, 카메라 착용자의 action 위주로 학습을 하게 된다
% We leverage an MLLM to provide environmental information, \ie detailed captions, to discriminate various contexts and thereby reduce the search space. + 새로운 loss에 대한 학습 방법을 제시한다. 

% 기존 웍들이 무엇을 하고 있는지 or 어떤 문제점이 있는지 -> 우리는 어떤걸 보여주면서 이걸 어떻게 해결하려고 하는지
% 짜잔 우리랑 관련 있는 웍들은 이런 이런 게 있습니다!! (x)
% 이런 이런 게 있는데 얘들은 여기를 태클 했고 쟤들은 저길 태클 했는데 아쉬운 부분이 어디어디가 있었다 그래서 우리는 여길 태클했다 (o)

% Video-language grounding(VLG)를 해결하기 위해 다양한 방법을 시도했다. 비디오의 탐색 범위를 줄이기 위해 proposal을 생성하거나(cpl, iron, cone), 입력으로 들어온 query에 있는 object를 파악하기 위해 object detector(helpinghands), training dataset의 부족함을 완화하기 위해 data augmentation을 이용하는(NaQ) 등의 방법이 있다. 이러한 다양한 시도가 있음에도 불구하고 proposal이 정확하지 않을 경우 최종 prediction 단계에서 올바르게 답을 맞추는데 어려움이 있다. 또한, egocentric video 상에서 카메라 착용자와 상호작용하는 object 위주로 파악하거나 매우 큰 데이터셋을 기반으로 pretraining을 진행해야 했다. 우리는 proposal을 생성하지 않고 탐색 범위를 줄이며 카메라 착용자와 상호작용하는 object 뿐만 아니라 주변 환경을 파악하며 large dataset 없이도 모델을 학습시킬 수 있는 방안을 제시하고자 한다.

% \textbf{Long-Form video-language grounding.} Various approaches have been attempted to solve long-form video-language grounding. These include generating proposals to reduce the search space\cite{Pan_2023_ICCV, Zheng_2022_CVPR, Cao_2023_CVPR, Mun_2020_CVPR}, using object detectors to identify objects mentioned in the query \cite{zhanghelpinghand}, using simulation datas \cite{nagarajan2023egoenv} and employing data augmentation to mitigate the lack of training data \cite{ramakrishnan2023naq, di2023groundvqa, linegocentric, liu2022reler}. We propose an approach that reduces the search space without generating proposal. We provides comprehensive details about the surrounding environment, not just the objects and this can help to reduce search space. Additionally, our method does not rely on large datasets for training.

% Long-term videos have become a vibrant research area with the advent of long-term video datasets~\cite{Soldan_2022_CVPR, ZhXuCoCVPR18, lei2021detecting} including Ego4D~\cite{grauman2022ego4d}.
% This work addresses the {\ltvlg} task known as EgoNLQ~\cite{grauman2022ego4d}.
% Existing approaches to video-language grounding (VLG) are categorized into three types:
% \begin{enumerate}
%     \item Structural approaches: iterative proposal calibration~\cite{Cao_2023_CVPR}, hierarchy~\cite{hou2023cone, hou2023groundnlq, Mun_2020_CVPR} % , Proposal generation
%     \item Additional information infusion: Data augment~\cite{ramakrishnan2023naq, Croitoru_2023_ICCV}, physical environment modeling~\cite{nagarajan2023egoenv}
%     \item Multi-task learning: Masked modeling~\cite{Zheng_2022_CVPR}, object detection~\cite{zhanghelpinghand}, VideoQA~\cite{di2023groundvqa}, reasoning~\cite{jang2023knowing}
% \end{enumerate}
% However, structural methods often produce false negatives due to a lack of physical experience, which is central to human cognition.
% For instance, proposal methods fail in long-term settings because the accuracy of the initial proposal is significantly low, leading to a high probability of error propagation.
% The ground truth moment coverage rates are very low: 27.0\% for Charades-STA~\cite{Gao_2017_ICCV} and only 2.3\% for EgoNLQ~\cite{grauman2022ego4d}.
% % EgoEnv 얘기는 related work 가서 하는 게 좋을까요?
% While EgoEnv\cite{nagarajan2023egoenv} suggested modeling the physical environment, its approach requires simulation construction, making it less accessible.
% We propose a method to convey human \textit{experience} to models through MLLMs, which have learned from a vast amount of prior knowledge.



% Large Language Model(LLM)이 발달함에 따라 videoQA(ex llovi)와 같은 multi-modal task에서 적용되고 있다. 그러나, MLLM은 VLG에서는 아직 좋은 성능을 보이지 못하고 있다(TimeChat, VTimeLLM) 따라서 우리는 MLLM 자체를 VLG task에 적용하기보다 large dataset으로부터 학습되었기 때문에 zero-shot이 가능하다는 점을 활용하여 주변 environment 정보를 얻는데 활용하려고 한다.

% Recently, MLLMs~\cite{
% li2023llavamed, liu2024llavanext, liu2024visual, liu2023improvedllava,
% zhang-etal-2023-video, lin2023video,
% li2022blip, li2023blip2, instructblip,
% ren2023timechat, maaz2023videochatgpt} built upon open-source LLMs~\cite{
% radford2018improving, radford2019language, NEURIPS2020_1457c0d6,
% touvron2023llama, touvron2023llama2,
% jiang2023mistral, jiang2024mixtral,
% vicuna2023, alpaca} have demonstrated superior zero-shot performance in various video tasks, including needle-in-a-haystack and VideoQA.
% % Flamingo(prop), VideoCoCa(prop?), VideoPrism(prop?)
% MLLMs can generate comprehensive explanations encompassing object detection and action recognition, even from short-term videos or single frames.
% Despite this, it is challenging for (M)LLMs to perform grounding.
% According to ~\cite{ren2023timechat, feng2023llm4vg, wang2024lifelongmemory, wang2023egocentric}, the grounding performance of LLMs is very low though tuned with instructions.
% While (M)LLMs excel at recalling and answering questions within an extensive sequence of tokens (needle-in-a-haystack) by remembering the necessary information,
% they struggle significantly with localizing the point where the information was found.

% \textbf{Multi-modal Large Language Models} With the advancement of Large Language Models (LLMs)\cite{vicuna2023, alpaca, touvron2023llama, touvron2023llama2}, these models have been applied to multi-modal tasks such as VQA \cite{zhang2023simple, liu2024visual, liu2024llavanext, maaz2023videochatgpt, li2023llavamed, lin2023video, liu2023improvedllava} and captioning \cite{huang2023vtimellm, instructblip}. However, in the task Video-Language Grounding (VLG), MLLMs \cite{ren2023timechat, huang2023vtimellm, wang2024lifelongmemory} have not yet demonstrated strong performance. Rather than applying MLLMs directly to the VLG task, we aim to leverage their zero-shot reasoning capability \hg{which cap?}, to extract detailed environmental information from the video.


% 기존에는 여러 긴 document에서 특정 information을 찾기 위해 sentencebert, cross-encoding 등과 같은 시도가 있었다. 즉, 긴 영상에서 특정 구간을 찾아야 하는 VLG task와 유사하다. 하지만,  infomation retrieval에서는 한 문서 안에서 내용을 구분하지 않지만, VLG task에서는 in-video clip에서 여러 environment를 구분해야 하는 점에서 차이가 있다. 우리는 여기서 단편적인 정보를 획득하는 것에서 확장하여 environment text information을 바탕으로 in-video clip 상에서 구분을 할 수 있도록 한다. 



% \textbf{Environment Features for {\ltvlg}.} Existing works have employed two main methods to provide information about the environment surrounding the camera wearer.\sy{cite egoenv} The first method involves training a model using simulation data, enabling the model to learn about the surrounding environment. However, this approach requires additional simulation data. 

% The second method involves dividing the long video into multiple short clips and using a captioner to describe each clip, thus providing environmental information.\sy{cite llovi, lifelongmemory} Although using a captioner pretrained on egocentric videos\cite{zhao2023lavila, islam2024video}, these models tend to focus on the camera wearer rather than the surrounding environment, making it difficult to obtain the necessary environmental information for solving NLQ. We propose to leverage MLLMs in a zero-shot manner to extract environmental information. This information is then used to train a text model that generates the final environment features, thereby improving the VLG task in long videos.



% \textbf{Reducing the search space by generating proposals.} To solve VLG in long videos, prior works\sy{cite cpl, cone, etc.} have focused on generating proposals that are likely to contain the answer, thereby reducing the search space. However, if these proposals are not accurate, it becomes challenging to make correct predictions in the final stage. We aim to enhance the VLG task by using information about the environment surrounding the camera wearer, which can help reduce the search space more effectively.

% 2. Env feature 생성하기
% 기존 웍은 어떻게 했지?
% - simulation data를 통해서 카메라 착용자에 대한 주변 env 정보 담기도록 model training
% - video captioner를 통해서 해당 구간마다 text를 통해 비디오에 대한 정보를 얻고자 했음
% 어떤 문제가 있지?
% - simulation data가 필요함
% - egocentric video로부터 학습된 captioner의 경우 environment를 묘사하기 보다 카메라 착용자를 중심으로 묘사하게 됨
% - NLQ를 풀기 위해서는 카메라 착용자에 대한 정보 뿐만 아니라 카메라 착용자가 있는 주변 환경에 대한 정보가 있어야 함
% - 하지만, 기존 웍대로 NLQ를 풀게 되면 충분한 정보를 바탕으로 문제를 푸는게 아니기 때문에 
% 우리는 어떻게 해결할까?
% - simulation data 사용하지 않아도 됨
% - LLM으로부터 env 묘사하도록 하게 함
% - 이를 통해서 text model을 학습시킨 뒤 text? Text feature?만을 이용하여 env 정보 제공하고자 함
% - 주변 환경까지 잘 이해하도록 LLM을 통해 environment에 대한 정보를 획득하고 이를 기반으로 text model을 학습시켜 env 정보를 잘 제공하려고 함
% 언급할만한 논문: Egoenv, llovi, lifelongmemory
% 기존 work에서는 egocentric 비디오에서 카메라 착용자 주변에 대한 environment 정보를 제공하기 위해 두 가지 방법을 이용했다.  첫번째로 simulation data를 이용하여 model을 training하여 모델이 주변 environment에 대해 학습하는 방법이다. 이 방법의 경우 추가로 simulation data가 필요하다는 문제점이 있다. 두번째 방법은 long video를 여러 개의 짧은 clip으로 나눠서 captioner를 통해 해당 clip을 묘사하여 environment 정보를 제공하는 방법이다. 그러나, egocentric video로 pretrained된 captioner를 사용할 경우 주변 environment를 묘사하는 것이 아닌 camera wearer를 중심으로 묘사한다. 즉, NLQ를 풀기 위한 camera wearer의 주변 environment 정보를 획득하기 어렵다. 우리는 MLLM을 이용하여 zero-shot을 통해 environment 정보를 획득한 뒤 이를 기반으로 text model을 학습시켜 최종 environment feature를 생성하도록 한다.





==> 3_overview.tex <==
\section{Overview}
\label{sec:overview}

% Introduce your problem with a toy example

% This figure illustrate the overall process of the algorithm, starting from inputs, processing steps, and outputs. Use forward references the figures with the corresponding equations and sections in the paper.
% \input{figure/5_fig_overview}

\hg{Problem Def?}

==> figure/fig_motivation.tex <==
\begin{figure}[t]
\centering
    % \includegraphics[width=\textwidth]{img_files/blank.png}
    \jbox{\textwidth}{0.3\linewidth}
    \figcaption{Motivation}{What is the main motivation of this paper?}
    \label{fig:motivation}
\end{figure}

==> table/_ablation.tex <==
\begin{table*}[t]
\centering
\caption{\tb{Ablation study.}
We show results from an R(2+1)D ResNet-34 model on the 20\% label split of the UCF-101 dataset.
\jw{This is a placeholder for the main table. Please replace it according to your project.}
}

\mpage{0.34}{(a) Temporally-coherent photo.-geo. aug.}\hfill
\mpage{0.30}{(b) Temporal augmentation}\hfill
\mpage{0.32}{(c) ActorCutMix augmentation}\hfill
\\
%% Color and spatial
\mpage{0.32}{
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
Strategy & Top-1 acc. \\
\midrule
Supervised baseline & 38.91 \\
\midrule
Per-frame & 44.17 \\
Temporally-coherent & \textbf{53.37} \\
\bottomrule
\end{tabular}
}
}
%% Temporal aug
\mpage{0.32}{
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
Strategy & Top-1 acc. \\
\midrule
T-Half & 42.77 \\
T-Drop & 43.14 \\
T-Reverse & 43.40 \\
\midrule
TemporalAll & \textbf{44.07} \\
\bottomrule
\end{tabular}
}
}
%% Label smoothing for ACM
\mpage{0.32}{
\resizebox{1.05\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
Strategy & Detection & Top-1 acc. \\
\midrule
% Supervised baseline & - & 38.91 \\
Sup. baseline & - & 38.91 \\
\midrule
w/o smoothing & \cite{he2017mask} & 42.82 \\
w/ smoothing & \cite{he2017mask} & \textbf{45.28} \\
\midrule
% w/ unsupervised detector & Unsup. & 45.12 \\
w/ unsup. det. & \cite{yang2019unsupervised} & 45.12 \\
\bottomrule
\end{tabular}
}
}
\\
\vspace{2mm}

\mpage{0.30}{(d) Combining intra-clip augs.}
% photo.-geo. and temporal augmentations}\hfill
\mpage{0.38}{(e) Combining intra- and cross-clip augs.}\hfill
% \mpage{0.29}{(f) Different initialization}\hfill
\mpage{0.29}{(f) Different SSL frameworks}\hfill
\\
%% RandAug + TempAug
\mpage{0.32}{
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
Strategy & Top-1 acc. \\
\midrule
Supervised baseline & 38.91 \\
\midrule
Randomly sample one & 53.37 \\
Cascaded & \textbf{54.48} \\
\bottomrule
\end{tabular}
}
}
\hfill
%% Combination
\mpage{0.32}{
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
Strategy & Top-1 acc. \\
\midrule
Supervised baseline & 38.91 \\
\midrule
Cascaded & 50.89 \\
Randomly sample one & \textbf{56.73} \\
\bottomrule
\end{tabular}
}
}
\hfill
%% Semi-Supervised Learning Frameworks
\mpage{0.32}{
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
% & \multicolumn{2}{c}{Semi-supervised framework} \\
% \cmidrule{2-3}
Method & FixMatch & UDA \\
\midrule
Vanilla & 44.17 & 43.11 \\
Vanilla+temp.-co. & 53.37 & 50.20 \\
Ours & \textbf{56.73} & \textbf{54.80} \\
\bottomrule
\end{tabular}
}
}
\label{tab:abl}
\end{table*}


==> table/_main_all.tex <==
\begin{table*}[htbp]
\centering
\caption{\tb{Comparison with the state of the arts.}
\jw{This is a placeholder for the main table. Please replace it according to your project.}
}

\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
& w/ ImageNet & Kinetics-100 && \multicolumn{4}{c}{UCF-101} && \multicolumn{3}{c}{HMDB-51}\\
\cmidrule{3-3}
\cmidrule{5-8}
\cmidrule{10-12}
Method & distillation & 20\% && 50\% & 20\% & 10\% & 5\% && 60\% & 50\% & 40\% \\
\midrule
PseudoLabel~\cite{lee2013pseudo} & - 
& 48.0
&& 47.5 & 37.0 & 24.7 & 17.6
&& 33.5 & 32.4 & 27.3
\\
MeanTeacher~\cite{tarvainen2017mean} & - 
& 47.1 
&& 45.8 & 36.3 & 25.6 & 17.5
&& 32.2 & 30.4 & 27.2
\\
S4L~\cite{zhai2019s4l} & - 
& 51.1 
&& 47.9 & 37.7 & 29.1 & 22.7 
&& 35.6 & 31.0 & 29.8
\\
VideoSSL~\cite{jing2020videossl} & \checkmark 
& {57.7} 
&& {54.3} & {48.7} & \second{42.0} & \second{32.4}
&& {37.0} & {36.2} & {32.7}
\\
Ours & - 
& \second{61.2} 
&& \second{59.9} & \second{51.7} & {40.2} & {27.0}
&& \second{38.9} & \second{38.2} & \second{32.9}
\\
Ours & \checkmark 
& \best{68.7} 
&& \best{64.7} & \best{57.4} & \best{53.0} & \best{45.1}
&& \best{40.8} & \best{39.5} & \best{35.7}
\\
\bottomrule
\end{tabular}
}

% \label{tab:main_all}
\end{table*}


==> table/abalation_v2.tex <==
% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l c cccc}
% \toprule
% & \textbf{R1@0.3} & \textbf{R5@0.3} & \textbf{R1@0.5} & \textbf{R5@0.5}
% \\
% \midrule
% \textit{with all components} \\
% \midrule
% {\ours}  & 15.2 & 35.2 & 10.0 & 23.8 \\  % 버전: 102720
% % \;w/ VideoRecap\cite{islam2024video} & 15.0 & 34.5 & 9.6 & 23.5 \\
% \;w/ VideoRecap & 15.0 & 34.5 & 9.6 & 23.5 \\
% % \;w/ LLaVA video 7B\cite{liu2024llavanext} & 15.4 & 34.5 & 10.0 & 23.6 \\
% \;w/ LLaVA video 7B & 15.4 & 34.5 & 10.0 & 23.6 \\
% \;w/o Env cues  & 15.3 & 34.3 & 9.4 & 23.4 \\
% \;Concat. $\rightarrow$ Add & 14.9 & 34.6 & 9.9 & 23.5 \\
% \;Concat. $\rightarrow$ CA & 15.2 & 34.4 & 9.8 & 23.3 \\ 
% \midrule
% \textit{VSLNet Probe} \\
% \midrule
% {\ours}
% & 8.0 & 14.2 & 4.6 & 8.9 \\  % 버전: 102720
% % EgoEnv~\cite{nagarajan2023egoenv}
% EgoEnv
% & 7.7 & 14.0 & 4.6 & 9.0 \\
% \midrule
% \textit{Text-Only Probe} \\
% \midrule
% {\ours} & 1.5 & 7.3 & 0.5 & 2.8 \\
% {\ours} & 1.8 & 7.6 & 0.8 & 3.0 \\  %        / all-MiniLM-L6-v2  / 성무진 교수님
% {\ours} & 1.5 & 7.7 & 0.4 & 2.8 \\  % 104454 / all-MiniLM-L6-v2  / 성무진 교수님 reproduce
% \;Loss: \\
% \;\;MLL $\rightarrow \emptyset$ & 1.4 & 5.7 & 0.5 & 2.0 \\
% \;\;MLL $\rightarrow$ BCE & 1.5 & 6.4 & 0.6 & 2.5 \\
% % \;Text-model: EgoVLP\cite{linegocentric} & 1.8 & 7.3 & 0.6 & 2.8 \\
% \;Text-model: \\
% \;\;SBERT $\rightarrow$ EgoVLP & 1.8 & 7.3 & 0.6 & 2.8 \\
% \bottomrule
% \end{tabular}
% }
% \caption{\tb{Ablation study.}}
% \label{tab:abl_v2}
% \end{table}


% \begin{table}[h]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l c cccc}
% \toprule
% & \textbf{R1@0.3} & \textbf{R5@0.3} & \textbf{R1@0.5} & \textbf{R5@0.5}
% \\
% \midrule
% {\ours}  & 15.2 & 35.2 & 10.0 & 23.8 \\  % 버전: 102720
% % \;w/ VideoRecap\cite{islam2024video} & 15.0 & 34.5 & 9.6 & 23.5 \\
% \;w/ VideoRecap & 15.0 & 34.5 & 9.6 & 23.5 \\
% % \;w/ LLaVA video 7B\cite{liu2024llavanext} & 15.4 & 34.5 & 10.0 & 23.6 \\
% \;w/ LLaVA video 7B & 15.4 & 34.5 & 10.0 & 23.6 \\
% \;w/o Env cues  & 15.3 & 34.3 & 9.4 & 23.4 \\
% \;Concat. $\rightarrow$ Add & 14.9 & 34.6 & 9.9 & 23.5 \\
% \;Concat. $\rightarrow$ CA & 15.2 & 34.4 & 9.8 & 23.3 \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{\tb{Ablation study of \mj{blahblah}}}
% \label{tab:abl_v2}
% \end{table}

% \begin{table}[h]
% \centering
% \resizebox{0.8\columnwidth}{!}{
% \begin{tabular}{l c cccc}
% \toprule
% & \textbf{R1@0.3} & \textbf{R5@0.3} & \textbf{R1@0.5} & \textbf{R5@0.5}
% \\
% \midrule
% {\ours}
% & 8.0 & 14.2 & 4.6 & 8.9 \\  % 버전: 102720
% % EgoEnv~\cite{nagarajan2023egoenv}
% EgoEnv
% & 7.7 & 14.0 & 4.6 & 9.0 \\
% \bottomrule
% \end{tabular}
% }
% \caption{\tb{Ablation study of \mj{blahblah}}}
% \label{tab:abl_v2}
% \end{table}

% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l c cccc}
% \toprule
% & \textbf{R1@0.3} & \textbf{R5@0.3} & \textbf{R1@0.5} & \textbf{R5@0.5}
% \\
% \midrule
% {\ours} & 1.5 & 7.3 & 0.5 & 2.8 \\
% {\ours} & 1.8 & 7.6 & 0.8 & 3.0 \\  %        / all-MiniLM-L6-v2  / 성무진 교수님
% {\ours} & 1.5 & 7.7 & 0.4 & 2.8 \\  % 104454 / all-MiniLM-L6-v2  / 성무진 교수님 reproduce
% \;Loss: \\
% \;\;MLL $\rightarrow \emptyset$ & 1.4 & 5.7 & 0.5 & 2.0 \\
% \;\;MLL $\rightarrow$ BCE & 1.5 & 6.4 & 0.6 & 2.5 \\
% % \;Text-model: EgoVLP\cite{linegocentric} & 1.8 & 7.3 & 0.6 & 2.8 \\
% \;Text-model: \\
% \;\;SBERT $\rightarrow$ EgoVLP & 1.8 & 7.3 & 0.6 & 2.8 \\
% \bottomrule
% \end{tabular}
% }
% \caption{\tb{Ablation study of \mj{blahblah}}}
% \label{tab:abl_v2}
% \end{table}

==> table/ablation.tex <==
\begin{table*}[t]
\centering
Before revision by Jinwoo
\caption{\tb{Ablation study.}
We show results comparing various design choices.
(a) and (b) are trained on the VSLNet with backbones frozen.
We report text-only scores in (c).
\jw{Please update caption accordingly ASAP.}
}

% \mpage{0.49}{(a) GroundVQA vs. ours}\hfill
% \mpage{0.49}{(b) Comparison of information quality. Reproduced\textsuperscript{*}.}\hfill
%\\
%% vs. gfoundvqa
\mpage{0.49}{
% \subcaption{GroundVQA vs. ours}
\subcaption{Effect of environment cues.}
\label{tab:abl_groundvqa}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l c cccc}
\toprule
Method && R1@0.3 & R5@0.3 & R1@0.5 & R5@0.5 \\
\midrule
w/o environment cues\textsuperscript{\textdagger}
&& 15.3 & 34.3 & 9.4 & 23.4 \\
% \midrule
% EgoEnv~\cite{nagarajan2023egoenv}\textsuperscript{*}
% && 8.46 & 14.32 & 4.75 & 9.58 \\
w/ environment cues
&& 15.2 & 35.2 & 10.0 & 23.8 \\  % 버전: 102720
\bottomrule
\end{tabular}
}
}
%% vs. EgoEnv (VSLNet)
\mpage{0.49}{
% \subcaption{Comparison of information quality.Reproduced\textsuperscript{*}}
\subcaption{Quality of environment cues.}
\label{tab:abl_egoenv}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l c cccc}
\toprule
Method && R1@0.3 & R5@0.3 & R1@0.5 & R5@0.5 \\
\midrule
EgoEnv~\cite{nagarajan2023egoenv}\textsuperscript{*}
&& 7.7 & 14.0 & 4.6 & 9.0 \\
% \midrule
% EgoEnv~\cite{nagarajan2023egoenv}\textsuperscript{\textdagger}
% && 8.46 & 14.32 & 4.75 & 9.58 \\
Ours
&& 8.0 & 14.2 & 4.6 & 8.9 \\  % 버전: 102720
\bottomrule
\end{tabular}
}
}
\\
% \vspace{2mm}

% \mpage{0.49}{(a) Comparison of information quality. Reported\textsuperscript{\textdagger}, Reproduced\textsuperscript{*}.}\hfill
% \mpage{0.49}{(c) vs. Ego4D captioner}\hfill
% \mpage{0.49}{(d) Choices of the text model. (text-only metric)}\hfill
% \\
% vs. Ego4D captioner (VSLNet)
\mpage{0.49}{
% \subcaption{vs. Ego4D captioner}
\subcaption{Effect of caption quality.}
\label{tab:abl_ego4d_captioner}
\resizebox{.95\linewidth}{!}{
\begin{tabular}{l c cc c cccc}
\toprule
Caption generator && Zero-shot? & Stride && R1@0.3 & R5@0.3 & R1@0.5 & R5@0.5 \\
\midrule
VideoRecap~\cite{islam2024video}
&& - & 2s && 15.0 & 34.5 & 9.6 & 23.5 \\
LLaVA video 7B Env\jw{cite}
&& \checkmark & 2s && 15.4 & 34.5 & 10.0 & 23.6 \\
LLaVA image 34B Env\jw{cite}
&& \checkmark & 10s && 15.2 & 35.2 & 10.0 & 23.8 \\  % 102720
\bottomrule
\end{tabular}
}
}
\mpage{0.49}{
\subcaption{Effect of text encoder.}
\label{tab:abl_text_model}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l cccc}
\toprule
Text encoder & R1@0.3 & R5@0.3 & R1@0.5 & R5@0.5 \\
\midrule
% SentenceBERT & cosine
% && 1.52 & 7.32 & 0.46 & 2.75 \\  % 이효건 버전
EgoVLP-text\jw{cite}
& 1.80 & 7.33 & 0.62 & 2.75 \\
SentenceBERT\jw{cite}
& 1.82 & 7.56 & 0.77 & 2.97 \\  % 성무진 교수님 버전
\bottomrule
\end{tabular}
}
}
\\
% \vspace{2mm}

% \mpage{0.49}{(e) Effect of various losses for fine-tuning the text-model.}\hfill
% \mpage{0.49}{(f) Architecture of Environment Infuser.}\hfill
% \\
%% sbert fine-tune, hist (Text-only)
\mpage{0.49}{
\subcaption{Effect of text encoder learning.}
\label{tab:abl_losses}
\resizebox{0.70\linewidth}{!}{
\begin{tabular}{l c cccc}
\toprule
Method && R1@0.3 & R5@0.3 & R1@0.5 & R5@0.5 \\
\midrule
Frozen   && 1.41 & 5.71 & 0.48 & 1.96 \\         %        / all-mpnet-base-v2
BCE && 1.45 & 6.41 & 0.62 & 2.53 \\         % 102612 / all-mpnet-base-v2
MLL (Ours) && 1.52 & 7.32 & 0.46 & 2.75 \\
MLL (Ours) && 1.82 & 7.56 & 0.77 & 2.97 \\  %        / all-MiniLM-L6-v2  / 성무진 교수님
MLL (Ours) && 1.47 & 7.71 & 0.42 & 2.83 \\  % 104454 / all-MiniLM-L6-v2  / 성무진 교수님 param대로 reproduce
\bottomrule
\end{tabular}
}
}
%% Architecture of Injection
\mpage{0.49}{
\subcaption{Environment infuser architecture.}
\label{tab:abl_environment_infuser}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l c cccc}
\toprule
Architecture && R1@0.3 & R5@0.3 & R1@0.5 & R5@0.5 \\
\midrule
Add && 14.9 & 34.6 & 9.9 & 23.5 \\  
Cross-attention && 15.2 & 34.4 & 9.8 & 23.3 \\
Concatenation (Ours) && 15.2 & 35.2 & 10.0 & 23.8 \\
\bottomrule
\end{tabular}
}
}
\label{tab:abl}
\end{table*}





